GreyConE: Greybox fuzzing+Concolic execution guided test generation for high level design

Exhaustive testing of high-level designs pose an arduous challenge due to complex branching conditions, loop structures and inherent concurrency of hardware designs. Test engineers aim to generate quality test-cases satisfying various code coverage metrics to ensure minimal presence of bugs in a design. Prior works in testing SystemC designs are time inefficient which obstruct achieving the desired coverage in shorter time-span. We interleave greybox fuzzing and concolic execution in a systematic manner and generate quality test-cases accelerating test coverage metrics. Our results outperform state-of-the-art methods in terms of number of test cases and branch-coverage for some of the benchmarks, and runtime for most of them.

==> 3_problemAndmotivatingEg.tex <==
\section{Motivating case-study}
\label{sec:limitAndChallenge}
% We present our motivating case-study on a real-time finite state machine implementation. We use a system controller design mimicking a typical hardware functionality and highlight limitations of existing techniques to discover the trojan behavior.

% \subsection{Motivating case-study}
In~\autoref{label:motivatingCode}, we have a simple code-snippet that reads an integer from a file input and checks its divisibility by $2$ and $3$ with all possible checkings in $4$ branches. At $Branch~1$ and $Branch~4$, the program checks whether the number is divisible by both $2$ and $3$ or not. At $Branch~2$ and $Branch~3$, it checks if the number is divisible by either $2$ or $3$  thus giving a room to the test engines for different path exploration.
\lstinputlisting[caption=Motivating example,style=customc,label={label:motivatingCode}]{codes/motiv_exe.c}


\lstinputlisting[caption={Example showing symbolic Inputs},style=customc,label={label:symb_motive}]{codes/symb_in_eg.c}


\subsection{Evaluating AFL on this Example:}

We invoke fuzz engine AFL for fuzz testing the program with random input seeds. We continue running AFL for a time duration of two hours and measure the code coverage whenever a new test case is generated. AFL begins by generating interesting test inputs that take the program into a new path for a period of time but unable to reach certain portions of code with nested conditional branch statements. From the \texttt{LCOV} coverage report, it is observed that AFL failed to generate test cases that satisfies the complex checks at $Branch~1$ and $Branch~3$ of the program, covering $72.2\%$ of branches in the entire course of two hours time. AFL gets stuck at $662$ seconds, unable to generate any new test input exploring new paths. Thus we conclude our evaluation with a simple takeaway message: fuzzing needs additional aid to explore code segments guarded by complex conditional checks.

\subsection{Evaluating S2E on this example: }

We run S2E in pure symbolic mode on our motivating example with changes highlighted in~\autoref{label:symb_motive}. We use the $s2e\_make\_symbolic()$ function in order to specify the symbolic input for the program. It is interesting to observe that, S2E could attain $90\%$ of branch coverage traversing the path along $Branch~1$, $Branch~2$, and $Branch~3$ with its generated test cases. However, S2E takes a long time of $2186$ seconds and could not explore beyond line $14$ of~\autoref{label:symb_motive} in the set time duration. S2E calls the constraints solver at each conditional branch that depends on symbolic inputs in order to determine the feasibility of the outcomes. When a branch depends on symbolic data, symbolic execution does not know which branch outcome is feasible without calling the solver, thus sometimes getting lost in state space, taking longer time. 

To distinguish from pure symbolic execution, we also run S2E on our motivating example in concolic mode using initial random seed inputs. S2E attains a maximum branch coverage of $66.7\%$ covering only $Branch~1$ and $Branch~4$ beyond which it could not explore. The presence of \textit{while} loop in the program makes S2E to fork two states for every iteration of while loop soon running out of memory. On a high-level, it shows that concolic engines require an additional aid
for intelligent exploration of search space leaving less memory footprint. Performance of S2E in concolic mode depends on the quality of the concrete seeds provided. Thus, if the input seeds to S2E are coming from a fuzzer, it would drive the program down the path that reaches interesting parts of that program.
\subsection{Lessons learnt:} Evaluating with baseline techniques using vanilla AFL and naive S2E individually, we conclude that the main challenges lying ahead involve: generating high quality test cases attaining a target coverage metric in a scalable manner using less computation time and minimal resources. Our evaluation with fuzzing and concolic testing shows that they can be combined in a synergistic way to accelerate the test generation mechanism. Combining the two mainstream techniques for testing, GreyConE can achieve high code coverage. GreyConE avoids getting stuck either in fuzz testing or in symbolic execution. \emph{GreyConE} can avoid the path explosion problem of symbolic execution to a certain extend, by controlled forking in symbolic loops using the fuzzer-generated test cases.

\begin{figure*}[h]
\begin{center}
\includegraphics[width=1.55\columnwidth]{images/new_GreyConE_framework.png}
\end{center}
\caption{\emph{GreyConE} test generation framework --- \emph{Fuzz engine} is fed with initial test-cases and \emph{Concolic engine} starts as soon as a new test-case is detected via fuzzer. Test-cases are fed back and forth between \emph{Fuzz engine} and \emph{Concolic engine} to accelerate the search space exploration. The \emph{Coverage Calculator} checks for target coverage whenever \emph{GreyConE} generates a new test-case.} 
%The beta version of the implementation reported here does not include the shaded arrows from Concolic engine to Fuzz engine, and Fuzz engine to Trojan Detector}
\label{fig:flow_chrt}
\end{figure*}

% This can avoid the path explosion problem of symbolic execution by controlled forking in symbolic loops using the fuzzer-generated test inputs, thereby reaching deeper code segments without generating lots of states.

{\small
\begin{algorithm}[!ht]
\footnotesize
\SetAlgoLined
\KwData{Instrumented Design Under Test $DUT_{ins-exe}$, User provided test-inputs $T_{initial}$, User defined time bound $time_{cut-off}$} %\Comment{Design Under Test (DUT)}

%\Comment{$T_{initial}$, user provided test-input}

%$TC\gets$ $\pi$\; 
%$Q$ $\gets$ $\emptyset$\;
\KwResult{{$T_{fuzzed}$}       
   \Comment{Interesting test-inputs queue}}
$T_{fuzzed} \gets T_{initial}$ \Comment{Initialization of the AFL's test-inputs queue}\\ 
%$T_{new} \gets \phi$\\
%$T_{queue} \gets T_{initial}$\\
\While{time $ \leq time_{cut-off}$}{
    \For{$\tau \in T_{fuzzed}$} 
   {
        \Comment{Mutate $\tau$ to generate test-cases based on the energy parameter}\\
        $K\gets$ CALCULATE\_ENERGY($\tau$)\\
        \For{$i \in \{1,2,\dots,K\}$}{
            $\tau'\gets$ MUTATE-SEED($\tau$) \Comment{$\tau'$ denotes the mutated test case} \\
            \If{IS-INTERESTING($DUT_{ins-exe}, \tau'$)}
            {
            $T_{fuzzed}\gets$ $T_{fuzzed}\cup \tau'$
            \Comment{$\tau'$ is interesting if it improves branch coverage}\\}
           % {
        %    continue\;
        %    }
        }
        % \For{i from 0 to l}{
        %     $t'\gets$ MUTATE_SEED($T$)
        }
    %    $T_{fuzzed} \gets T_{fuzzed}$
    }
    \Return $T_{fuzzed}$
\caption{FUZZER($DUT_{ins-exe}$, $T_{initial}$)}
\label{algo:AFL_FUZZ}
\end{algorithm}
}

% {\small
% \begin{algorithm}[!ht]
% \SetAlgoLined
% \KwData{Design Under Test $DUT$, User provided test-inputs $T_{initial}$, $Time_{cut-off}$} %\Comment{Design Under Test (DUT)}

% %\Comment{$T_{initial}$, user provided test-input}

% %$TC\gets$ $\pi$\; 
% %$Q$ $\gets$ $\emptyset$\;
% \KwResult{$T_{fuzzed}$} 
% $T_{fuzzed} \gets T_{initial}$\\ 
% %$T_{new} \gets \phi$\\
% %$T_{queue} \gets T_{initial}$\\
% \While{time $ \leq Time_{cut-off}$}{
%     \For{$\tau \in T_{fuzzed}$}{
%         $K\gets$ CALCULATE\_ENERGY($\tau$)\\
%         \For{$i \in \{1,2,\dots,K\}$}{
%             $\tau'\gets$ MUTATE-SEED($\tau$) \\
%             \If{IS-INTERESTING($DUT, \tau'$)}
%             {
%             $T_{fuzzed}\gets$ $T_{fuzzed}\cup \tau'$
%             }
%           % {
%         %    continue\;
%         %    }
%         }
%         % \For{i from 0 to l}{
%         %     $t'\gets$ MUTATE_SEED($T$)
%         }
%     %    $T_{fuzzed} \gets T_{fuzzed}$
%     }
% \Return $T_{fuzzed}$
% \caption{FUZZER ($DUT$, $T_{initial}$)}
% \label{algo:AFL_FUZZ}
% \end{algorithm}
% }


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

